AR You on Track? Investigating Effects of Augmented Reality Anchoring on Dual-Task Performance While Walking

With the increasing spread of AR head-mounted displays suitable for everyday use, interaction with information becomes ubiquitous, even while walking. However, this requires constant shifts of our attention between walking and interacting with virtual information to fulfill both tasks adequately. Accordingly, we as a community need a thorough understanding of the mutual influences of walking and interacting with digital information to design safe yet effective interactions. Thus, we systematically investigate the effects of different AR anchors (hand, head, torso) and task difficulties on user experience and performance. We engage participants (n=26) in a dual-task paradigm involving a visual working memory task while walking. We assess the impact of dual-tasking on both virtual and walking performance, and subjective evaluations of mental and physical load. Our results show that head-anchored AR content least affected walking while allowing for fast and accurate virtual task interaction, while hand-anchored content increased reaction times and workload.

==> content/03_concept.tex <==
\section{Concept}
\label{sec:concept}


==> img/plot_answerrate_answertime.tex <==
\begin{figure*}[th!]

	\includegraphics[width=\linewidth]{img/plots/sumplot_acorrect_atime.pdf}

    \vspace{-1em}

	\begin{minipage}[t]{.45\linewidth}
		\centering
%        \includegraphics[width=\linewidth]{img/plots/plot_AnswerTime.pdf}
		\subcaption{\dvAnswerTime{} }\label{fig:results:AnswerTime}
	\end{minipage}%
    \begin{minipage}[t]{.45\linewidth}
		\centering
%        \includegraphics[width=\linewidth]{img/plots/plot_CorrectAnswerRate.pdf}
		\subcaption{\dvCorrectAnswerRate{}}\label{fig:results:GEQ}
	\end{minipage}%
	\caption{The mean results for (a) \dvAnswerTime{} and (b) \dvCorrectAnswerRate{} as a bar chart plot. The error bars indicate the standard error.}
	\Description[TODO]{TODO}
	\label{fig:plot_answertime_rate}
\end{figure*}

==> img/plot_prefAnchoring.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/plots/plot_prefAnch.pdf}
    \caption{PLACEHOLDER: Do we want to keep this? Preferred anchoring in different tasks}
    \label{fig:plot_prefAnch}
\end{figure}

==> img/study_procedure.tex <==
% A "teaser" image appears between the author and affiliation
% information and the body of the document, and typically spans the
% page.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/met/procedure.pdf}
    \caption{Experiment Procedure.}
    \label{fig:procedure}
\end{figure}

==> img/tables/data_sum_nback.tex <==
\begin{table*}
\centering
\caption{Mean Values (M) and Standard Deviation (SD) for the virtual \nback{n} task for the \dvAnswerTime{}, \dvAccuracy{} and \dvMissedAnswerRate{} (Missed AR).}
\Description{A table providing an overview of the Mean Values and Standard Deviation of the virtual nback task data analysis.}
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}{lllrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Answer Time} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{Missed AR} \\
\cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
Walking Task & Difficulty & Anchoring & M & SD & M & SD & M & SD\\
\midrule
No Walking & 1-back & Hand & .97 & .38 & .95 & .21 & .02 & .13\\
No Walking & 1-back & Head & .97 & .42 & .95 & .22 & .02 & .15\\
No Walking & 1-back & Torso & .94 & .37 & .94 & .24 & .02 & .15\\
No Walking & 2-back & Hand & 1.27 & .53 & .87 & .33 & .03 & .16\\
No Walking & 2-back & Head & 1.18 & .46 & .85 & .36 & .07 & .25\\
No Walking & 2-back & Torso & 1.22 & .55 & .87 & .34 & .04 & .19\\
\addlinespace
Walking & 1-back & Hand & 1.16 & .42 & .90 & .30 & .02 & .15\\
Walking & 1-back & Head & 1.09 & .40 & .92 & .28 & .02 & .14\\
Walking & 1-back & Torso & 1.29 & .56 & .90 & .31 & .02 & .14\\
Walking & 2-back & Hand & 1.43 & .57 & .78 & .41 & .06 & .24\\
Walking & 2-back & Head & 1.38 & .60 & .81 & .39 & .06 & .24\\
Walking & 2-back & Torso & 1.60 & .68 & .76 & .43 & .09 & .28\\
\bottomrule
\end{tabular}}
\end{table*}

==> img/tables/data_sum_subjective.tex <==
\begin{table*} %[t!]
\centering
\caption{Mean Values (M) and Standard Deviation (SD) for the TLX and the Median and Median Absolute Deviation (MAD) for the statements "My Performance on the Virtual Task Was Very Successful" (VP) and "It was hard to Focus on the Virtual Task" (HFVT).}
\Description{A table providing an overview of the Mean Values and Standard Deviation of the TLX data, as well as the Median and Median Absolute Deviation for two Likert items.}
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}{lllrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{TLX} & \multicolumn{2}{c}{VP} & \multicolumn{2}{c}{HFVT} \\
\cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
Walking Task & Difficulty & Anchoring & M & SD & Median & MAD & Median & MAD\\
\midrule
No Walking & 1-back & Hand & 3.94 & 2.82 & 7.0 & 0.00 & 2.0 & 1.48\\
No Walking & 1-back & Head & 3.02 & 2.47 & 7.0 & 0.00 & 1.0 & 0.00\\
No Walking & 1-back & Torso & 2.97 & 1.98 & 7.0 & 0.00 & 2.0 & 1.48\\
No Walking & 2-back & Hand & 5.51 & 3.36 & 6.0 & 1.48 & 2.5 & 2.22\\
No Walking & 2-back & Head & 5.12 & 3.20 & 6.0 & 1.48 & 2.0 & 1.48\\
No Walking & 2-back & Torso & 5.49 & 2.88 & 6.0 & 1.48 & 3.0 & 2.22\\
\addlinespace
Walking & 1-back & Hand & 6.44 & 3.58 & 6.0 & 1.48 & 5.0 & 2.97\\
Walking & 1-back & Head & 5.30 & 3.42 & 6.0 & 1.48 & 3.0 & 1.48\\
Walking & 1-back & Torso & 5.86 & 3.50 & 6.0 & 1.48 & 3.0 & 2.22\\
Walking & 2-back & Hand & 8.26 & 3.32 & 5.0 & 1.48 & 5.0 & 1.48\\
Walking & 2-back & Head & 7.71 & 3.59 & 5.5 & 0.74 & 5.0 & 2.97\\
Walking & 2-back & Torso & 8.29 & 3.68 & 5.0 & 2.22 & 3.5 & 2.22\\
\bottomrule
\end{tabular}}
\end{table*}

==> img/tables/data_sum_walking_PERC.tex <==
\begin{table}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}{llrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Walking Error} & \multicolumn{2}{c}{Stride Duration} & \multicolumn{2}{c}{Stride Length} & \multicolumn{2}{c}{Stride Width} & \multicolumn{2}{c}{Walking Speed} \\
\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8} \cmidrule(l{3pt}r{3pt}){9-10} \cmidrule(l{3pt}r{3pt}){11-12}
Difficulty & Anchoring & M & SD & M & SD & M & SD & M & SD & M & SD\\
\midrule
1-back & Hand & 11.18 & 71.47 & 14.58 & 73.91 & -2.72 & 73.10 & 6.27 & 37.33 & -16.07 & 35.04\\
1-back & Head & 7.52 & 71.41 & 13.66 & 69.97 & 0.21 & 76.23 & 4.09 & 38.98 & -13.39 & 33.44\\
1-back & Torso & 7.49 & 70.50 & 22.27 & 82.13 & 2.67 & 75.84 & 3.25 & 38.55 & -19.72 & 34.33\\
2-back & Hand & 10.78 & 70.72 & 17.61 & 76.57 & -2.48 & 72.27 & 2.48 & 36.74 & -17.19 & 39.39\\
2-back & Head & 9.74 & 72.22 & 15.52 & 76.78 & -0.08 & 74.19 & 7.93 & 48.99 & -12.40 & 36.45\\
2-back & Torso & 8.91 & 72.08 & 22.86 & 114.76 & 0.44 & 73.58 & 2.10 & 35.10 & -20.07 & 30.00\\
\bottomrule
\end{tabular}}
\caption{Mean values (M) and Standard Deviation (SD) of the walking data analysis. All values are relative to the baseline and in \%.}
\end{table}

==> img/walkingpath123.tex <==
\begin{figure*}[th!]
    %\vspace{2em}
	%\includegraphics[width=\linewidth]{img/plots/sumplotIOS_GEQ_TLX.pdf}

    \vspace{-1em}
	\begin{minipage}[t]{.48\linewidth}
		\centering
        \includegraphics[width=\linewidth]{img/met/walkingpath1.pdf}
		\subcaption{}
        \label{fig:walkingpath1-3}
	\end{minipage}%
    \hfill
    \begin{minipage}[t]{.48\linewidth}
		\centering
        \includegraphics[width=\linewidth]{img/met/walkingpath2.pdf}
  		\subcaption{}
        \label{fig:walkingpath2-3}
	\end{minipage}%
    \newline
     \begin{minipage}[t]{.48\linewidth}
		\centering
        \includegraphics[width=\linewidth]{img/met/walkingpath3.pdf}
		\subcaption{}
        \label{fig:walkingpath3-3}
	\end{minipage}%
	\caption{A top view schematic of the walking area. The width is 6.8m and the height 3.4m. The light blue elements show the path generation during the experiment. (a) The participant starts at the first node and sees the first two path sections. (b) Once the participant reaches the second node, the next path section lights up. (c) After the reaching the next node, the next path section illuminated and the second to last section turns off. This continuous to ensure that before reaching the node, the path section behind the node is already illuminated.}
	\Description[TODO]{A figure consisting of three TODO}
	\label{fig:walkingpath123}
\end{figure*}

